Analyzing privacy-aware mobility behavior using the evolution of spatio-temporal entropy

Analyzing mobility behavior of users is extremely useful to create or improve existing services. Several research works have been done in order to study mobility behavior of users that mainly use users' significant locations. However, these existing analysis are extremely intrusive because they require the knowledge of the frequently visited places of users, which thus makes it fairly easy to identify them. Consequently, in this paper, we present a privacy-aware methodology to analyze mobility behavior of users. We firstly propose a new metric based on the well-known Shannon entropy, called spatio-temporal entropy, to quantify the mobility level of a user during a time window. Then, we compute a sequence of spatio-temporal entropy from the location history of the user that expresses user's movements as rhythms. We secondly present how to study the effects of several groups of additional variables on the evolution of the spatio-temporal entropy of a user, such as spatio-temporal, demographic and mean of transportation variables. For this, we use Generalized Additive Models (GAMs). The results firstly show that the spatio-temporal entropy and GAMs are an ideal combination to understand mobility behavior of an individual user or a group of users. We also evaluate the prediction accuracy of a global GAM compared to individual GAMs and individual AutoRegressive Integrated Moving Average (ARIMA) models. These last results highlighted that the global GAM gives more accurate predictions of spatio-temporal entropy by checking the Mean Absolute Error (MAE). In addition, this research work opens various threads, such as the prediction of demographic data of users or the creation of personalized mobility prediction models by using movement rhythm characteristics of a user.

==> dataset_used.tex <==
\section{Dataset}
\label{sec:dataset}

The datasets used in this research work comes from two data collection campaigns: \emph{Nokia dataset}, presented in \cite{Laurila2012TheMD}, and \emph{Breadcrumbs dataset}.
These two datasets were chosen because they contain locations of users and other additional data extremely interesting to understand their mobility behavior, more specifically demographic data of users.\\ 

\noindent\textbf{Nokia dataset.}
Nokia dataset was collected from March 2009 to March 2011 in the Lake Geneva region.
This data collection campaign was organized by the Nokia Research Center of Lausanne, Swiss Federal Institute of Technology in Lausanne (i.e., EPFL) as well as Idiap research institute.
In terms of data, each user dataset contains location traces from GPS and WLAN, mobile application usage, sms and call number and duration, and much more.
In addition, some users have demographic data such as mainly gender, age group and working profile.
There are exactly 153 users having all the three demographic data mentioned above.
However, the user datasets contains a lot of gaps from several hours to several days.
We decided to select the richest user datasets to analyze them for our research goals and only 14 user met our requirements in terms of dataset quality.
Each selected user has a very low number of successive days without any location, i.e., lower than 3 days, as well as a dataset period of more than 20 days.
Additional data is also available for these users, such as data related to application usage on their mobile devices, sms and calls.
The majority of the 14 users has a very long dataset duration up to~500 days for some of them.\\

\noindent\textbf{Breadcrumbs dataset.}
Breadcrumbs dataset is a data collection campaign that started at the end of March 2018 and finished at the end of June 2018 in the Lake Geneva region, at the University campus of Lausanne more specifically.
The motivation behind this data collection campaign was to obtain rich user datasets having a rich regularity in terms of location tracking: at least one location per hour in the best case as well as a ground truth of points of interest validated by the users themselves.
For this research work, we used 48 users having very rich location history of at least 20 days and at least only three days without any location.
The duration of their datasets is between 31 and 34 days.
Because the data collection campaign was in progress during the period of the analysis, we could only obtain this dataset duration.
The added value of this dataset compared to the Nokia dataset is that there is a higher location frequency tracking per day.
Every user dataset has a rich location history with a high accuracy as well as a detailed an additional dataset containing demographic data that can give additional valuable information about the mobility behavior of the user, such as transportation means used, family status, and much more.\\

%\noindent To summarize, these two datasets are complementary because \emph{Nokia dataset} allows us to have 14 rich user datasets over a long period of time, while \emph{Breadcrumbs dataset} enables to have 48 users with rich ...

==> demographic_data_prediction.tex <==
\section{Towards demographic data prediction}
\label{sec:towards_emographic_data_prediction}

%After having analyzed Figure~\ref{fig:summary_global_GAM_48users} that is describing the effects on the co-variables on the spatio-temporal entropy of the 48 users of the \emph{Breadcrumbs} dataset.
%We can now check if it would be possible to do the opposite: seeing the effect of the spatio-temporal entropy on the demographic variable itself using a GaM for categorical response data.

This research analysis opens a various number of future works, which can be focused on demographic data prediction of users.
We discuss about this topic in this section.
First, it is extremely important to introduce a new dataset in order to motivate this new research work.
The \emph{Breadcrumbs} dataset 

\subsection{Nokia dataset}

Nokia dataset was collected from March 2009 to March 2011 in the Lake Geneva region.
This data collection campaign was organized by the Nokia Research Center of Lausanne, Swiss Federal Institute of Technology in Lausanne (i.e., EPFL) as well as Idiap research institute.
In terms of data, each user dataset contains location traces from GPS and WLAN, mobile application usage, sms and call number and duration, and much more.
In addition, some users have demographic data such as mainly gender, age group and working profile.
There are exactly 153 users having all the three demographic data mentioned above.
However, the user datasets contains a lot of gaps from several hours to several days.
We decided to select the richest user datasets to analyze them for our research goals and only 14 user met our requirements in terms of dataset quality.
Each selected user has a very low number of successive days without any location, i.e., lower than 3 days, as well as a dataset period of more than 20 days.
Additional data is also available for these users, such as data related to application usage on their mobile devices, sms and calls.
The majority of the 14 users has a very long dataset duration up to~500 days for some of them.\\

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
